Multi-Sensor Event Detection using Shape Histograms

Vehicular sensor data consists of multiple time-series arising from a number of sensors. Using such multi-sensor data we would like to detect occurrences of specific events that vehicles encounter, e.g., corresponding to particular maneuvers that a vehicle makes or conditions that it encounters. Events are characterized by similar waveform patterns re-appearing within one or more sensors. Further such patterns can be of variable duration. In this work, we propose a method for detecting such events in time-series data using a novel feature descriptor motivated by similar ideas in image processing. We define the shape histogram: a constant dimension descriptor that nevertheless captures patterns of variable duration. We demonstrate the efficacy of using shape histograms as features to detect events in an SVM-based, multi-sensor, supervised learning scenario, i.e., multiple time-series are used to detect an event. We present results on real-life vehicular sensor data and show that our technique performs better than available pattern detection implementations on our data, and that it can also be used to combine features from multiple sensors resulting in better accuracy than using any single sensor. Since previous work on pattern detection in time-series has been in the single series context, we also present results using our technique on multiple standard time-series datasets and show that it is the most versatile in terms of how it ranks compared to other published results.

==> sec/3-RelatedWork-old.tex <==
Detecting events of interest in time-series data has been studied in many different application domains. Initial work explored a variety of
methods and classifiers based on statistics and machine learning theory. Guralnik and Srivastava \cite{Guralnik:1999} addressed the time
series event detection as a change detection problem by modelling the time-series using a piecewise segmented model. Early work by Rodriguez
et al. \cite{rodriguez00learning} introduced inductive logic programming for multivariate time-series classification as well as the
application of boosting for improving the performance of the resulting classifiers. A knowledge-based event detection framework for
time-series arising in health monitoring systems is discussed in \cite{Hunter99knowledge}. Other approaches include using recurrent neural
networks for time-series classification by organizing the network dynamics in alignment with class labels (Husken and Stagge
\cite{HuskenS03}).

Availability of sufficient labelled data is important aspect of time-series classification problem. In this context, Wei and Keogg \cite{Wei:2006} presented semi-supervised learning using nearest neighbour time-series classification with insufficient labelled data. 

Xi et al. \cite{Xi:2006} proposed a dynamic-time-warping-based nearest neighbour classifier for addressing time complexity in case of large datasets. Recently
Jeong et al. \cite{Jeong2011} presented weighted dynamic time warping for time-series classification by associating higher weights to phase differences in local neighbourhood.

In summary, each of the above methods concentrated on experimentation with different classifiers and similarity measures. However, they did not adequately address real-time requirements of time and space complexity. In \cite{Ye:2009}, Ye and Keogg introduced `shapelet' based time-series classification, where a shapelet is a time-series sub-sequence considered as maximal representative of a class. Information-gain based shapelet discovery locates the most informative local pattern for classification using linear search over the complete time-series. Subsequently a decision tree is defined on the computed information gains to perform the time-series classification. 

In an extension of shapelet based time-series analysis, Mueen et al. \cite{Mueen:2011} proposed logical combination of multiple shapelets for performance improvement. Lines et al. \cite{Lines:2012} extended the shapelet concept for transforming the time-series in uniform data space so as to be able
to use other classifiers in addition to decision trees. The \textit{k} best shapelets extracted from the data in combination with decision tree classifier were shown to achieve comparable performance with the results presented in \cite{Ye:2009}. 
 
In further extensions of the shapelet idea of local pattern analysis, Zakaria et al. \cite{Zakaria2012} proposed unsupervised learning based shapelet discovery method for clustering time-series subsequences. The underlying philosophy is the creation of min-dist based distance map between a local pattern (read unsupervised shapelet), and set of time-series subsequences.

Note that the shapelet discovery algorithms discussed in \cite{Ye:2009,Mueen:2011,Lines:2012} all require apriori label information: in other words,
they require labelled data to calculate the shapelet descriptors themselves, rather than just for the classification stage. In contrast our shape histogram feature descriptor can be computed independent of the events to be detected. 

Most of the above pattern detection techniques deal with detecting fixed-length waveform patterns. Shapelets, however, do treat variable-length patterns as does our shape histogram approach; therefore our experimental comparisons in Section \ref{Sec_ER} are primarily with the shapelet approach, especially on our real-life vehicular data where variable length events are indeed present.

At the same time, since the shapelet descriptors are themselves of variable length this restricts their use in conjunction with state-of-the art machine learning classifiers such as SVMs; in contrast, shape histograms do not have this restriction. (Note that this advantage that is also shared by the shapelet-transform extension by Lines et al. \cite{Lines:2012}.)



==> sec/PublicDatasets.tex <==
\subsubsection{Gun-point dataset}
The Gun-point dataset \cite{RatanamahatanaK04} consists of hand-motion patterns of an actor depicting gun drawing action from a hip mounted holster, gun-pointing at the target for approximately one second and returning to normal state. 
The dataset has been widely applied for evaluation of many frameworks for time-series analysis. 
Patterns in the dataset describe two categories representing real and fake gun pulling action, each having 100 example instances. Each instance has sequences of 150 values, where each value represent X-axis co-ordinate of the centroid of actor's right hand tracked for the entire action sample uniformly over. 
The standard partitioning of the dataset is done as 50 instances in training and 150 instances in testing set. Note that in this and other public datasets, the candidate sequences are of fixed length. The results of the evaluation is presented below.

\subsubsection{Coffee dataset}
The Coffee dataset \cite{Lines:2012} consists of spectrograph samples of two widely produced coffee types. The complete dataset consists of 56 examples, uniformly distributed between training and testing having 28 examples each. While the training set has balanced distribution of two categories, the testing set has 15/13 distribution between two categories. 
Recent results on this dataset have yielded perfect classification results \cite{Lines:2012}. Shape histogram based classification also achieved perfect results as shown in Table \ref{Tb_GunPoint}.
\subsubsection{Face (four) dataset}
The Face dataset is a collection of pseudo time series data converted by head profile of four different individuals making different expressions such as talking, smiling, laughing, frowning etc. \cite{Face_dataset}. In this context, time-series represent the local angle of its perimeter trace starting from the neck area. 
The complete collection consists of 112 instances having 350 points with training and testing partitioning as 24, and 88 examples each, the task being to classify head pose. 
Using shape histograms computed with 36 distance bins and 90 orientation bins, euclidean distance based 1-nearest neighbour achieved 92.73\% accuracy. 
For the same descriptor setting 1-vs-all SVM with RBF kernel achieved 96.73\% accuracy. Mean precision, and recall measures are also presented in the Table \ref{Tb_GunPoint}.
\subsubsection{Wafer dataset}
Wafer dataset include measurements of a vacuum-chamber sensor during the etch process of silicon wafer manufacture \cite{Wei:2006}. After the processing, each wafer is classified as normal or abnormal. In the complete set of 7164 data-streams of sensor measurements, 762 are identified as abnormal. Train and test partitioning have been done as provided on \cite{dataset:Keogg} where training set contains 97 abnormal and 903 normal wafer time-series. The classification objective here was to identify the data-streams corresponding to normal/abnormal wafers. With shape descriptor computed with 50 distance bins and 45 orientation bins, RBF kernel based SVM achieved 99.68\% classification accuracy. The mean precision, and recall measures are presented in the Table \ref{Tb_GunPoint}.
\subsubsection{SonyAIBORobot Surface dataset}
This dataset contains accelerometer data-streams of a SONY AIBO Robot dog walking on two different surfaces: carpet and cement. Only X-axis readings have been considered where each data-stream correspond to one robot walk having 70 measurements \cite{dataset:Keogg}. 
Training set contains of 20 data-streams of partitioned as 6/14. Test set contains 601 instances distributed as 343/248 with the objective to identify the surface of the walk. 
Noisy data, and small training set poses complex 2-category classification problem. With shape histogram for 35 distance bins and 15 orientation bins, RBF kernel based SVM achieved 91.54\% accuracy. 
With combination of Shapelets, 96.34\% accuracy has been reached. Nevertheless, with average occupancy of 8.23\%, computational complexity of analysis 

\subsubsection{SonyAIBORobot SurfaceII dataset}
This is another dataset having accelerometer recordings of SONY AIBO Robot dog walking on different surfaces with each walk having 65 measurements \cite{dataset:Keogg}. Here, the training set contains of 27 data-streams of distributed as 11/16. 
Whereas, the test set contains 953 instances distributed as 365/588 with similar classification objective to identify the surface of the walk. In this dataset, shape histogram computed with 25 distance, and 10 orientation bins, RBF kernel based SVM achieved 88.88\% accuracy.   
\subsubsection{Beef dataset}
The dataset contains 60 data-streams of spectrogram measurements having pure and adulterated beef with varying degrees of offal \cite{BagnallDHL12}. Each data-stream is 470 values long belonging to one of the five distinct categories based on the quality. Training and testing set contain 30 data-streams each. Classification objective is identification of the quality. Using shape histogram computed with 45 distance and 10 orientation bins, with 1-Vs-1 SVM classifier RBF kernel achieved 73.33\% accuracy. 
\subsubsection{OliveOil dataset}
Similar to Beef dataset, this dataset contains 60 data-streams of spectrogram measurements of Oliveoil belonging to four classes. Here, a class denote the geographic origin of the olive oil \cite{BagnallDHL12}. Each data-stream in 570 values long, with training and testing set having uniformly distribution of 30 examples each. The shape histogram computed with 40 distance and 36 orientation bins achieved 80\% accuracy with 1-Vs-1 SVM classifier with RBF kernel. 
\subsubsection{Trace dataset}
This dataset is a subset of synthetic dataset designed to simulate the instrumentation failures in a nuclear power plant \cite{Roverso00}. The original dataset consists of 16 classes, 50 instances in each class with each instance having 4 features. 
Nevertheless, this dataset available at \cite{dataset:Keogg} is compiled with only second feature of class 2 and 6, and second feature of class 3 and 7 \cite{RatanamahatanaK04}. 
The subset contains 200 instances, 50 for each class with each instance having 275 values. 
Training and testing set are partitioned with 100 instances each. Shape histogram computed with 35 distance and 36 orientation bins with 1-vs-1 SVM with RBF kernel achieved perfect classification as shown in the Table \ref{Tb_GunPoint}. Our result matches with result of other recent methods on this dataset \cite{Lines:2012}. 
\subsubsection{ECG dataset}
Electrocardiogram (ECG) dataset contains measurements of cardiac electrical activity as recorded
from electrodes at various locations on the body. Each data-stream in the dataset has the measurements recorded by one electrode during one heartbeat \cite{Olszewski:2001}. All of the data-streams have been normalized to vector having 96 values, and have a label of normal or abnormal as annotated by domain expert. The complete collection contains 200 data-streams of which 133 are identified as normal and 67 as abnormal. With 40 distance bins and 45 orientation bins, the RBF kernel based SVM achieved 91.35\% accuracy which is comparable with the results reported in \cite{BagnallDHL12}.  
\subsubsection{Lightning-2 dataset}
This dataset has a collection of 121 data-streams distributed as 60/61 in training and testing set. Each data-stream is a vector of 637 length having a binary label. Existing results on this dataset have reported classification accuracy between 78.70 ~ 87.89\% \cite{Lin:2007,4634188}. Whereas, using shape histogram computed with 40 distance and 36 orientation bins in combination with RBF-SVM, we achieve 88.64\% accuracy.    
\subsubsection{Lightning-7 dataset}
Lightning-7 dataset consists of 143 time-series of satellite recordings of transient electromagnetic events associated with lightning. Each data-stream is 319 values long, associated with an event (label) described by the physical characteristics of the stream. Existing compilation of the dataset has stream belonging to seven distinct events \cite{libsvmDE02a}.
Using shape histogram with RBF-SVM, we achieve 64.38\% accuracy in correctly identifying the lightning type which is comparable with other state-of-the-art \cite{Lines:2012}.  

\subsubsection{ItalyPowerDemand dataset}
The dataset consists of 67 train and 1029 test time-series having 24 values describing per day, average per hour power demand in Italy from the period of January to June. Here, the classification objective is to predict the quarter (January-March, April-June) of the recorded power-demand time-series.
In particular, the dataset poses unique challenge, as in the same class, i.e., quarter, power demand varies significantly from weekdays to holidays. 
Also, similarity in weather pattern in continuous months would influence similar power demand pattern in March and April. Using the shape histogram with different parameter settings, 36 distance and 36 orientation bins achieved classification accuracy of 90.74\% with 1-NN. 
For the same histogram parameters, RBF-SVM classifier trained with cost parameter C = 90, and standard deviation = 6.4 achieved accuracy of 94.28\% which is comparable/better than the results reported by other recent methods \cite{Lines:2012}. 
\subsubsection{MedicalImages dataset}
The MedicalImages dataset available at \cite{dataset:Keogg} poses 10-category classification problem of data-streams having 99 values. Data-streams are the pixel intesity histograms of medical images with each class represent different human body region. Training and testing set are partitioned as 381 and 760 instances. 
In object recognition research, several methods have been proposed for this particular problem. Using the time-series approach, with shapelet transform and linear SVM, the authors reported an accuracy of 52.50\% on this dataset \cite{Lines:2012}. The shape histogram computed with 40 distance and 36 orientation bins with 1-Vs-Rest SVM with RBF kernel obtained an accuracy of 58.98\% showing an improvement of 6.48\%.   
\subsubsection{FacesUCR dataset}
The FacesUCR dataset is a collection of the instances of 14 face images transformed into time-series. The time-series data represents the local angle of the perimeter trace of face images starting from the neck \cite{dataset:Keogg}. The collection has 2250 images from 14 individuals under different conditions including variety of expressions, and with/without eyeglasses. 
Each time-series is normalized to 131 time units, with training data having 200 instances. 
The problem is particularly complex because of variations in head angle, expressions with some wearing eyeglasses. 
With tree-ensemble classifier and interval features, Deng et al. reported accuracies between 87.13 $\sim$ 89.90\% with different split criterion \cite{Deng:2013}. The shape histogram computed 25 distance and 60 orientation bins, RBF-SVM achieved 86.56\% which is 4.64\% less than the best result reported on \cite{dataset:Keogg}.
\subsubsection{DiatomSizeReduction dataset}
This dataset has a collection of diatom images in pseudo time series form \cite{dataset:Keogg}. The objective of this dataset is to explore the distribution of shapes and valve face features of diatoms in morphospace. 
The collection has images from 4 taxa, i.e, classes. The collection has 16 training and 306 testing instances. 
Each time-series has a sequence of 345 values. 
In the existing works, different algorithms have reported accuracies between 56.54 $\sim$ 93.46 because of reasons such as small training set, 
and change in the scale of diatoms. With the shape histogram and 1-Vs-1 RBF-SVM, we achieved a classification accuracy of 91.88\%.   
\subsubsection{ChlorineConcentration dataset}
Chlorine concentration dataset consists of data-streams having the measurement of chlorine concentration level in a water network \cite{Li:2009}. The measurements are captured at 166 pipe junctions generating equally long time-series. 
This 3-class dataset has 467 training and 3840 testing instances. Using shape histogram computed with 30 distance and 30 orientation bins, 1-Vs-1 SVM with RBF kernel achieved classification accuracy of 64.18\%.
\subsubsection{Adiac dataset}
Adiac dataset consists of 781 daitom contour-streams of 37 taxon types, i.e, classes \cite{Adiac_2005}. Each taxon type, signifies a species or variety, has at least 20 representatives. Each data-streams has 176 values. Training and testing set are partitioned as 390 and 391 instances. On this dataset, we achieved 28.25\% classification accuracy with shape histogram computed with 25 distance and 36 orientation bins, and 1-vs-1 RBF-SVM. 
We see the application of Random Forest classifier with shapelet transform achieved an accuracy of 30.69\% \cite{Lines:2012}. Nevertheless with same descriptor, application of different classifiers have reported accuracies between 23.79 $\sim$ 30.43\%.
\subsubsection{SyntheticControl dataset}
This dataset contains 600 examples of synthetically generated control charts \cite{Alcock99}. A control pattern is a time-series showing the machine parameter variation with respect to time. There are six different classes of control charts generated by six different equations. Each time-series is 60 values long, with training and testing set having equal number of instances. Here, with shape histogram descriptor, and 1-Vs-1 SVM with RBF kernel, we achieve the best classification accuracy of 77.33\%. 
\subsubsection{SwedishLeaf dataset}
This dataset consists of 1125 Swedish leaf images converted in the time-series form by measuring the distance of contour points of the image with respect to its centroid \cite{Xi:2006}. The dataset has 15 classes of image, with training and testing set partitioned as 500, and 625. Shape histogram in the present case does not show a promising result with best accuracy of 74.53\% whereas other methods have shows much better results \cite{Xi:2006}. 
\subsubsection{Symbols dataset}
Symbols is a 6-class dataset having 25 training and 995 testing instances. Each instance is a data-series generated by X or Y-axis trace of the freehand drawing of a given symbol by a volunteer \cite{dataset:Keogg}. Each data-series has 398 values. There are 3 symbols, generating 6 different classes by individual labelling of X, and Y-axis traces. This poses a complex challenge for classification, because, even for different symbols, individual traces exhibit significant similarity. Existing works on this dataset have reported classification accuracy between 47.14 - 92.26\% \cite{Ye:2009,Lines:2012}. In this case, the shape histogram with 1-Vs-1 SVM with RBF kernel achieved an accuracy of 90.31\% which comparable with many recent time-series classification methods. 
\subsubsection{TwoLeadECG dataset}
This dataset poses heartbeat classification task in two classes, i.e., normal/abnormal. The dataset consists of 23 training and 1139 testing instances of 82 length. Classification on this dataset is challenging task because of subtle distinctions between samples from two classes, and very small training set. With shape histogram computed with 36 distance and 36 orientation bins, 1-NN based classification achieved 91.87\% accuracy. For the same histogram parameters, RBF-SVM achieved 99.56\% accuracy which is comparable with results of other recent methods \cite{Ye:2009,Lines:2012}. 
\subsubsection{MoteStrain dataset}
This data is a collection the month long recording of 48 Mote sensors installed in a lab environment. In this dataset, we have recording from two different sensors, i.e., two classes, having 20 training and 1252 testing instances. 
The streams are in z-normalized form having vector of 84 values. In particular, streams have large inter-class variations with many zeros because of drop-outs. With shape histogram based classification, our approach yielded an accuracy of 82.73\%. 
This is less accurate than the other reported results on this dataset \cite{Ye:2009,Lines:2012}. However, the reported results in this paper are based on SVM classifier, and we have explored other classifiers with shape histogram descriptor. 
\subsubsection{ECGFiveDays dataset}
ECGFiveDays dataset has a collection of ECG data series of a single patient recorded on the duration of five days. Each data series is annotated as either normal, or abnormal. The collection consists of 23 training, and 861 testing instances, with each series having 136 values. With the given training and testing set distribution, several methods have reported more than 98\% accuracy with the best of 99.88\% in \cite{Ye:2009}. Using shape histogram with 27 distance and 40 orientation bins we achieved an accuracy of 99.64\% with average occupancy of 6.14\%.

==> sec/related.tex <==
\section{Related works} \label{Sec_RW}
Interesting event detection in sensor data has been much studied data mining problem in context of different application domains. Initial works have explored variety of methods and classifiers based on statistics and machine learning theory. Guralnik and Srivastava \cite{Guralnik:1999} addressed the time series event detection as statistics theory based change detection problem by modelling the time-series using piecewise segmented model. Early work by Rodriguez et al. \cite{rodriguez00learning} introduced inductive logic programming based multivariate time-series classification. Subsequently, the application of boosting is demonstrated for improving the performance of resulting classifiers. Knowledge based event detection framework for time-series from health monitoring systems is discussed in \cite{Hunter99knowledge}. Availability of sufficient labelled data is important aspect of time-series classification problem. In this context, Wei and Keogg \cite{Wei:2006} presented semi-supervised learning using nearest neighbour time-series classification with insufficient labelled data. Xi et al. \cite{Xi:2006} proposed warping constraints in dynamic time warping based nearest neighbour classifier for addressing time complexity in case of large datasets. Husken and Stagge \cite{HuskenS03} applied the dynamics of Recurrent neural network for time-series classification by organizing the network dynamics in alignment with class labels. In \cite{Jeong2011}, Jeong et al. presented weighted dynamic time warping for time-series classification by associating higher weights to phase differences in local neighbourhood. In summary, these methods concentrated on experimentation with different classifiers as well as similarity measures. In \cite{Ye:2009}, Ye and Keogg introduced the concept of shapelets which are the time-series sub-sequences defined as maximal representative of a class. Information gain based shapelet discovery method is described which locates most informative local pattern for classification by linear search over the complete time-series. Decision tree is defined on the computed information gains is proposed for time-series classification.

The approach locates most informative local pattern for classification by linear search over the complete time-series using information theoretic criterion. Subsequently, Zakaria et al. \cite{Zakaria2012} proposed novel extension in local pattern based time-series analysis by proposing unsupervised shapelets for clustering application. The underlying philosophy is creation of a distance map based on min-dist between a local pattern (read unsupervised shapelet) and time-series sequence. Another interesting extension in this direction is discussed in \cite{Mueen:2011}, which proposes logical combination of multiple shapelets for scalability and improved performance. Lines et al. \cite{Lines:2012} extended the concept for extracting k best shape-lets by a parameter-free approach which could be directly applied with different classifiers for time series classification. In this work, we propose novel feature representation for time-series patterns using existing theory of shape based object representation. The representation provides uniform length representation to patterns of varying length and
% ------------------------------------------------------------------------------------------------------
% ------------------------------------------------------------------------------------------------------

